Constructing a Minimum-Level Phylogenetic Network from a Dense Triplet Set in Polynomial Time

For a given set $\mathcal{L}$ of species and a set $\mathcal{T}$ of triplets on $\mathcal{L}$, one wants to construct a phylogenetic network which is consistent with $\mathcal{T}$, i.e which represents all triplets of $\mathcal{T}$. The level of a network is defined as the maximum number of hybrid vertices in its biconnected components. When $\mathcal{T}$ is dense, there exist polynomial time algorithms to construct level-$0,1,2$ networks (Aho et al. 81, Jansson et al. 04, Iersel et al. 08). For higher levels, partial answers were obtained by Iersel et al. 2008 with a polynomial time algorithm for simple networks. In this paper, we detail the first complete answer for the general case, solving a problem proposed by Jansson et al. 2004: for any $k$ fixed, it is possible to construct a minimum level-$k$ network consistent with $\mathcal{T}$, if there is any, in time $O(|\mathcal{T}|^{k+1}n^{\lfloor\frac{4k}{3}\rfloor+1})$. This is an improved result of our preliminary version presented at CPM'2009.

==> Introduction.tex <==
\section{Introduction}
A triplet is a smallest rooted tree that contains evolutionary information. So, a classic problem is  to determine whether a given set of triplets is consistent with some phylogenetic tree, and if so, returning such a tree (Figure \ref{fig:combine_triplets}).
When the triplet set does not represent a tree-like evolution because of errors in data, or of hybridizations, recombinations,  lateral gene transfer events, then the problem becomes constructing phylogenetic networks that represent all triplets (Figure \ref{fig:combine_triplets_network}). Constructed networks allow us to see where are the conflicts, or the reticulate events. As mentioned in Section \ref{sec:phylogenetic_network}, there are many kinds of phylogenetic networks, the model in this problem is hybridization network.

\begin{figure}[ht]
\begin{center}
\subfigure[\label{fig:combine_triplets}]{\includegraphics[scale=.8]{Chapter4/Figures/combine_triplets.png}}
\subfigure[\label{fig:combine_triplets_network}]{\includegraphics[scale=.8]{Chapter4/Figures/combine_triplets_network.png}}
\caption{Combining triplets into a tree (a) or a network (b)}
\label{fig:combining_triplets}
\end{center}
\end{figure}

\cite{CJSS05} introduced a parameter for hybridization networks, called the \textit{level}, which is the number of hybridization vertices per biconnected component. The level of a network measures its distance to a tree, a level-$0$ network is indeed a tree, a level-$1$ network is a galled-network \cite{JNS06}. So, given a triplet set $\mathcal{T}$, and an integer $k$, one would like to construct a level-$k$ phylogenetic network which contains all these triplets.

\subsection{Some related works} 
Constructing phylogenetic networks from triplets is one of many combinatorial problems in phylogeny. 

\subparagraph*{Trees from triplets}
The first work of triplets is done by \cite{ASSU81}, the authors presented an $O(|\mathcal{T}|.n)$-time algorithm for determining whether a given set $\mathcal{T}$ of triplets is consistent with some rooted phylogenetic tree, and if so, returning such a tree. Divers implementation were given in \cite{GJLO98,HKW99,JNSS05}. If the set of triplet is \textit{dense}, \cite{GB10} presented a $O(n^3)$ algorithm which constructs a tree if there is any, and which exhibits a conflict otherwise. For the calculation of a tree from a dense triplet set after deleting a minimum number of $l$ leaves, \cite{GB10} proposed algorithms in $O(n^4+3.12^l)$ or $O(4^l.n^3)$, while the version without restriction of density is  NP-hard, and even W[2]-hard \cite{BN06}.

\subparagraph*{Networks from triplets}

The studies of triplets on phylogenetic networks began with the article of \cite{JS04} on level-$1$ networks, under the restriction that the triplet set is dense, i.e there is at least one triplet in the data for each three species. The authors gave a recursive structure of level-$1$ networks, as well as a recursive algorithm to construct a network which is implemented by dynamic programming. They introduced the notion of SN-set. This concept plays an important role in partitioning the leaf set such that each part is applied recursively by the algorithm. The problem is then polynomial for level-$1$ networks. \cite{BGHK08} proposed polynomial algorithms for constructing a level-$0,1,2$ network consistent with a part of the given triplet set.

- If there is no constraint on the triplet set, the problem  of constructing a level-$k$ phylogenetic network consistent with a triplet set is NP-hard for all $k$ greater than $0$ \cite{JNS06,IKKS08,IKM08}. 

- However, if the triplet set is dense, then the taxa set is better structured and then there are some positive results. As said above, \cite{JS04} gives a polynomial algorithm for level-$1$ networks.  After that, they authors improved the algorithm of calculating all SN-sets in $O(n^3)$ \cite{JNS06} which implies an $O(|\mathcal{T}|)$-time algorithm to construct a consistent network. \cite{IK08} gives an $O(n^5)$-time algorithm to construct a consistent one with the minimum number of reticulations. 

Latterly, \cite{IKKS08} gave a solution for level-$2$ networks. The solution is also based on SN-sets and recursive structure of networks, but explores a property of SN-sets on level-$2$ networks which replaces the one on level-$1$ networks. They proposed an implementation of the algorithm in time $O(|\mathcal{T}|^{\frac{8}{3}})$. The authors applied the algorithm to experimental data consisting of sequences from different isolates of a kind of yeast.
Then, \cite{IK08} presented an $O(n^9)$-time algorithm to construct the consistent one with the minimum number of reticulations. 

For level-$k$ networks with any fixed $k$, there was only a result constructing all simple networks in $O(|\mathcal{T}|^{k+1})$-time \cite{IK08}. We give a proof of the polynomiality of the problem in the general case of level-$k$ network \cite{TH09} and then an improvement result in \cite{HT11}.

However, when the level is unrestricted, it was recently proved in \cite{IK11} that the problem is NP-hard. Besides, an interesting recursive construction of level-$k$ phylogenetic networks was proposed in \cite{GBP09}.
Finding a network consistent with the maximum number of triplets is also NP-hard for all levels \cite{JNS06,IKM08}. 

- There are also studies on the version of extremely dense triplet sets, that is when $\mathcal{T}$ is considered to contain all triplets of a certain network. In this case, an $O(|\mathcal{T}|^{k+1})$ time algorithm was given in \cite{IK08} for level-$k$ networks. 

\subparagraph*{Other data}
Other problems consist of reconstructing phylogenetic trees or networks from a set of quartets, cluster or trees. 

- Reconstruction networks from trees having the same taxa set: 
Firstly, determining if a tree is contained in a network is NP-complete \cite{KNTX08}. %, même pour réseaux réguliers sans fratrie hybride. 
The problem is polynomial for normal networks, binary networks without hybrid descendants and level-$k$ networks \cite{ISS10}.

For $2$ trees, reconstruction a network with the minimum number of hybrid vertices is NP-complete and even APX-hard \cite{BS07b}.
The problem is FPT by the number of hybrid vertices \cite{BS07a,BLSS07,WW10}. However, if the trees are contained in a level-$1$ network having $k$ hybrid vertices, \cite{NWLS05} gave an $O(nk)$ algorithm.

\cite{Wu10} proposed an approach for more than $2$ trees. \cite{HJNS05} gave an $O(t^2n^2)$ algorithm to construct a network from $t$ rooted trees (not necessarily binary) whose a refinement is contained in a level-$1$ network.

Moreover, under some certain conditions, reconstruction a network with $h$ hybrid vertices from a species tree or a gene tree can be done in $O(2^{4h}n^2)$ (\cite{HL01,AHL03}).

Another direction of this problem is using consensus network to represent the tree set \cite{HM03}, which constructs median networks of dimension at most $k$. For heuristic approaches, \cite{NRW05,BH06,BPM2010} proposed algorithms to reconstruct networks with small number of hybrid vertices.

- Reconstruction trees or networks from quartets: As said in Chapter \ref{chap:pp}, constructing a tree from a quartet set is NP-complete \cite{BFW92,S92}. %, there is an approach (Chor,1998). 
If the quartet set is extremely dense, it is possible to reconstruct a tree with $O(n.logn)$ requests on the presence of a quartet \cite{KLW96}.
\cite{BB99} presented algorithms for phylogenetic construction from  weighted quartets.

If it is possible to obtain a tree containing the minimal quartet set after deleting $O(n)$ among them, then the problem is polynomial \cite{BJKLW99,WYL06}.

A variation of the problem is searching a maximum subset of  $\mathcal{Q}$ which is tree-like. This problem is introduced in \cite{BD86}, and then \cite{BG00} proposed a polynomial algorithm. 

\cite{GBP10} introduced a definition of level for unrooted phylogenetic networks which is coherent with the one for rooted phylogenetic network, and some results on this problem.

- Reconstruction networks from clusters: If we search a solution with the minimum number of hybrid vertices, the problem is NP-hard and even APX-hard \cite{IK11}. \cite{HRBGP09} proposed heuristic method and also an implementation for constructing galled networks from real data. \cite{IKRH10} gave another algorithm and model so that the constructed networks have smaller number of hybrid vertices. 

\subsection{Main results}
The following question was first asked  in \cite{JS06}: Given a dense triplet set $\mathcal{T}$. Can we determine if there exists a level-$k$ phylogenetic network consistent with $\mathcal{T}$, and construct one if there is any, in polynomial time for a fixed $k$?

We present an affirmative answer to this question. Our first result presented in \cite{TH09} is that we can construct a minimum level-$k$ network in time $O(|\mathcal{T}|^{k+1}n^{3k+1})$. After that, we improved the result to a complexity of $O(|\mathcal{T}|^{k+1}n^{\lfloor\frac{4k}{3}\rfloor+1})$. 

We propose the notion of split SN-set which is used to characterize the partition of the leaf set in a network. Then, by associating each split SN-set to some hybrid vertices, we can bound the number of split SN-set by the number of hybrid vertices in a block of the network, which is bounded by $k$. It returns to bound the number of possible partitions by a polynomial function of $k$. Several functions which assign for each split SN-set some hybrid vertices are defined and analysed in Section \ref{sec:split}. The properties of these functions are deduced from the definition of SN-set, of split SN-set and of consistency of each triplet with the network.

In Section \ref{sec:restrict}, we propose two lemmas which allow to restrict the research class and reduce the number of split SN-sets. We prove that, if a split SN-set satisfies some special condition, then we can modify the network so that it does not contain this split SN-set but remains consistent with the triplet set and keeps the same number of hybrid vertices. 

As a consequence, it is possible to find a network with the minimum level in polynomial time if the minimum level is restricted. It means that the complexity is a polynomial function with the power of the minimum level. 
